Multi-physics modeling of non-equilibrium phenomena in inductively coupled plasma discharges: Part II. Multi-temperature approach

This paper provides a comparison between the vibrational-specific state-to-state (StS) model for nitrogen plasma elaborated in Part I of this work and conventional two-temperature (2-T) models for simulating inductively coupled plasma (ICP) discharges under non-Local Thermodynamic Equilibrium (NLTE) conditions. Simulations are performed within the multi-physics computational framework established for ICP in Part I. Based on the findings of Part I, the quasi-steady-state (QSS) assumption is validated in the plasma core, thereby enabling the calculation of global rate coefficients under this assumption. This facilitates the reduction of the StS model to a "consistent" macroscopic 2-T model. Results from the StS model for nitrogen ICP torch exhibit considerable discrepancies when compared against predictions from the widely utilized Park 2-T model. On the contrary, the comparison between the newly proposed 2-T model, consistently derived from the original vibronic StS model, and the full StS results demonstrate excellent agreement in terms of plasma core location, morphology, and peak temperature distributions. This demonstrates the ability of the proposed 2-T model to capture the energy transfer and reactive processes predicted by the comprehensive StS model. Additionally, the study identifies the vibrational-translational (VT) energy transfer term in the 2-T model as the predominant factor in dictating plasma core morphology. This suggests a strong sensitivity of the ICP flow field to heavy-impact vibrational excitations and dissociative events.

==> compilePDF <==
#!/bin/bash

NAME="main"
TEX_FILE=$NAME.tex
PDF_FILE=$NAME.pdf
LOG_FILE=$NAME.log
AUX_FILE=$NAME.aux
BBL_FILE=$NAME.bbl

rm -f $LOG_FILE $AUX_FILE 

# Convert EPS files to PDF
#find Figures -name "*.eps" -exec epstopdf {} \;

# Compile LaTeX document
#pdflatex $TEX_FILE
#bibtex $NAME
#pdflatex $TEX_FILE
#pdflatex $TEX_FILE

# Compile LaTeX document with LuaLaTeX and --shell-escape flag
pdflatex --shell-escape $TEX_FILE
bibtex $NAME
pdflatex --shell-escape $TEX_FILE
pdflatex --shell-escape $TEX_FILE

rm -f $LOG_FILE $AUX_FILE


